Autoregressive Conditional Neural Processes

Conditional neural processes (CNPs; Garnelo et al., 2018a) are attractive meta-learning models which produce well-calibrated predictions and are trainable via a simple maximum likelihood procedure. Although CNPs have many advantages, they are unable to model dependencies in their predictions. Various works propose solutions to this, but these come at the cost of either requiring approximate inference or being limited to Gaussian predictions. In this work, we instead propose to change how CNPs are deployed at test time, without any modifications to the model or training procedure. Instead of making predictions independently for every target point, we autoregressively define a joint predictive distribution using the chain rule of probability, taking inspiration from the neural autoregressive density estimator (NADE) literature. We show that this simple procedure allows factorised Gaussian CNPs to model highly dependent, non-Gaussian predictive distributions. Perhaps surprisingly, in an extensive range of tasks with synthetic and real data, we show that CNPs in autoregressive (AR) mode not only significantly outperform non-AR CNPs, but are also competitive with more sophisticated models that are significantly more computationally expensive and challenging to train. This performance is remarkable given that AR CNPs are not trained to model joint dependencies. Our work provides an example of how ideas from neural distribution estimation can benefit neural processes, and motivates research into the AR deployment of other neural process models.

==> math.tex <==
% Define \charfusion. From https://tex.stackexchange.com/a/52673.
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
    \newcommand{\charfusion}[3][\mathord]{
        #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}}
        \ifx#1\mathop\expandafter\displaylimits\fi
    }
\makeatother

% Sha symbol.
%   Source: https://tex.stackexchange.com/questions/124738/i-just-want-to-write-sha-without-ruining-everything
\DeclareFontFamily{U}{wncy}{}
\DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
\DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
\DeclareMathSymbol{\Sha}{\mathord}{mcy}{"58}

% Define a bigger \cdot.
%   Source: https://tex.stackexchange.com/questions/235118/making-a-thicker-cdot-for-dot-product-that-is-thinner-than-bullet
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

% Bold math symbols from text greeks:
\newcommand{\mathbfup}[1]{\mathord{\textnormal{\textbf{#1}}}}

% Bold characters:
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\vecu}[1]{\hat{\vec{#1}}}
\newcommand{\mat}[1]{\vec{#1}}

% Predefined matrices and vectors:
\newcommand{\vnull}{\mathbf{0}}

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

% Must be enclosed in another group.
\newcommand{\vmu}{{\mathbfup{\textmu}}}
\newcommand{\vphi}{{\mathbfup{\textphi}}}
\newcommand{\vtau}{{\mathbfup{\texttau}}}
\newcommand{\vep}{{\mathbfup{\textepsilon}}}
\newcommand{\vth}{{\mathbfup{\texttheta}}}

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mK}{\mathbf{K}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mT}{\mathbf{T}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mZ}{\mathbf{Z}}

\newcommand{\mSigma}{\mathbfup{\textSigma}}

% Letters commonly used in blackboard bold font:
\newcommand{\Ab}{\mathbb{A}}
\newcommand{\Bb}{\mathbb{B}}
\newcommand{\Db}{\mathbb{D}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Hb}{\mathbb{H}}
\newcommand{\Jb}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Lb}{\mathbb{L}}
\newcommand{\Mb}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eR}{\overline{\mathbb{R}}}
\newcommand{\Sb}{\mathbb{S}}
\newcommand{\Tb}{\mathbb{T}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Z}{\mathbb{Z}}

% Letters commonly used in calligraphic font:
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\let\Haccent\H
\renewcommand{\H}{\mathcal{H}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\Jrat}{\mathcal{J}_{\text{rat}}}
\newcommand{\Kc}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Li}{\mathcal{L}{}^1}
\newcommand{\eLi}{\overline{\mathcal{L}}{}^1}
\newcommand{\m}{\text{m}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\eM}{\overline{\mathcal{M}}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

% Letters commonly used in sans serif font:
\newcommand{\T}{\text{\textsf{T}}}
\newcommand{\Ht}{\text{\textsf{H}}}
\renewcommand{\c}{\text{\textsf{c}}}

% Symbols:
\newcommand{\es}{\varnothing}
\newcommand{\e}{\varepsilon}
\newcommand{\sub}{\subseteq}
\renewcommand{\d}{\partial}
\renewcommand{\th}{\theta}
\newcommand{\Th}{\Theta}

% Substitute l for \ell throughout.
%   Source: https://tex.stackexchange.com/questions/1975/substituting-character-l-with-ell-throughout-math-mode
\mathcode`l="8000
\begingroup
\makeatletter
\lccode`\~=`\l
\DeclareMathSymbol{\lsb@l}{\mathalpha}{letters}{`l}
\lowercase{\gdef~{\ifnum\the\mathgroup=\m@ne \ell \else \lsb@l \fi}}%
\endgroup

% Convergence symbols:
\newcommand{\oto}[1]{\overset{#1}{\to}}
\newcommand{\uto}[1]{\underset{#1}{\to}}
\newcommand{\outo}[2]{\overset{#1}{\underset{#2}{\to}}}
\newcommand{\Lto}[1]{\oto{\L^{#1}}}
\newcommand{\weakto}{\rightharpoonup}
\newcommand{\distto}{\oto{\text{d}}}
\newcommand{\weakstarto}{\overset{\ast}{\rightharpoonup}}
% Big-O notation:
\renewcommand{\O}{O}

% Equality symbols:
\newcommand{\disteq}{\overset{\text{d}}{=}}

% Operators:
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\let\max\relax\DeclareMathOperator*{\max}{max}
\let\min\relax\DeclareMathOperator*{\min}{min}
\let\sup\relax\DeclareMathOperator*{\sup}{sup}
\let\inf\relax\DeclareMathOperator*{\inf}{inf\vphantom{p}}
\let\limsup\relax\DeclareMathOperator*{\limsup}{lim\,sup}
\let\liminf\relax\DeclareMathOperator*{\liminf}{lim\,inf\vphantom{p}}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\newcommand{\AC}{\operatorname{AC}}
\newcommand{\atan}{\operatorname{atan}}
\newcommand{\Breg}{\operatorname{D}}
\newcommand{\BV}{\operatorname{BV}}
\newcommand{\card}{\#}
\newcommand{\cconv}{\circledast}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\ch}{\operatorname{ch}}
\newcommand{\cliques}{\operatorname{cliques}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\col}{\operatorname{col}}
\newcommand{\comp}{\circ}
\newcommand{\contains}{\supseteq}
\newcommand{\conv}{\ast}
\newcommand{\cov}{\operatorname{cov}}
\renewcommand{\deg}{\operatorname{deg}}
\renewcommand{\det}{\operatorname{det}}
\newcommand{\diag}{\operatorname{diag}}
\renewcommand{\dim}{\operatorname{dim}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\dotcup}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\dotunion}{\charfusion[\mathop]{\bigcup}{\cdot}}
\newcommand{\dsum}{\oplus}
\newcommand{\Dsum}{\bigoplus}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\epi}{\operatorname{epi}}
\newcommand{\had}{\circ}
\newcommand{\Hell}{\operatorname{D}_{\text{Hell}}}
\newcommand{\hypo}{\operatorname{hypo}}
\newcommand{\im}{\operatorname{im}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\intersection}{\bigcap}
\newcommand{\join}{\lor}
\newcommand{\KL}{\operatorname{KL}}
\newcommand{\KOT}{\operatorname{KOT}}
\newcommand{\kron}{\otimes}
\newcommand{\len}{\operatorname{len}}
\newcommand{\Lip}{\operatorname{Lip}}
\newcommand{\meet}{\land}
\newcommand{\MOT}{\operatorname{MOT}}
\newcommand{\nullspace}{\operatorname{null}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\push}{_\#}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\rank}{\operatorname{rank}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\row}{\operatorname{row}}
\newcommand{\schur}{\operatorname{Schur}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sinth}{\operatorname{\sin\!\text{-}\Theta}}
\newcommand{\Sinth}{\operatorname{\text{Sin-}\Theta}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\symdiff}{\bigtriangleup}
\newcommand{\Tan}{\operatorname{Tan}}
\newcommand{\tensor}{\otimes}
\newcommand{\TV}{\operatorname{TV}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\union}{\bigcup}
\newcommand{\vecspan}{\operatorname{span}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\vol}{\operatorname{vol}}

% Probability distributions:
\newcommand{\Ber}{\operatorname{Ber}}
\newcommand{\Beta}{\operatorname{Beta}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\BM}{\operatorname{BM}}
\newcommand{\Cat}{\operatorname{Cat}}
\newcommand{\Cauchy}{\operatorname{Cauchy}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\Gam}{\operatorname{Gamma}}
\newcommand{\Geom}{\operatorname{Geom}}
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\InvWishart}{\mathcal{W}^{-1}}
\newcommand{\Laplace}{\operatorname{Laplace}}
\newcommand{\LogNormal}{\log\mathcal{N}}
\newcommand{\Mult}{\operatorname{Mult}}
\newcommand{\NegBin}{\operatorname{NegBin}}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\Poisson}{\operatorname{Poisson}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\Unif}{\operatorname{Unif}}
\newcommand{\Wishart}{\mathcal{W}}
\newcommand{\WN}{\operatorname{WN}}

\newcommand{\simiid}{\overset{\text{i.i.d.}}{\sim}}

% Probability commands:
\newcommand{\Var}{\V}
\newcommand{\Lik}{\L}
\newcommand{\iidsim}{\overset{\text{\tiny{i.i.d.}}}{\sim}}

% Special math commands:
\newcommand{\cond}{\,|\,}                  % Conditioning
\newcommand{\middlecond}{\,\middle|\,}     % Conditioning between a \left and \right
\newcommand{\divsep}{\,\|\,}               % Separator in divergences
\newcommand{\middledivsep}{\,\middle\|\,}  % Separator in divergences ebtween a \left and a \right

\newcommand{\sd}[1]{\mathrm{d} #1}         % Straight 'd'
\newcommand{\isd}[1]{\, \mathrm{d} #1}     % Straight 'd' in integral (with spacing)
% Straight 'd' in integral with spacing and absolute value around it
\newcommand{\asd}[1]{\, |\mathrm{d} #1|}

\newcommand{\idf}{\text{\textsf{id}}}      % Identity function
\newcommand{\sce}{\text{\sc{e}}}           % Scientific notation
\newcommand{\vardot}{\,\bigcdot\,}         % Variable dot
\renewcommand{\ss}[1]{_{\text{#1}}}        % Text subscripts
\newcommand{\us}[1]{^{\text{#1}}}          % Text superscripts

% Hard to type words:
\newcommand{\cadlag}{c\`adl\`ag}
\newcommand{\Cadlag}{C\`adl\`ag}
\newcommand{\ito}{It\^o}
\newcommand{\Ito}{\ito}
\newcommand{\levy}{L\`evy}
\newcommand{\Levy}{\levy}

% Subscripts
\newcommand{\loc}{_{\text{loc}}}
\newcommand{\lip}{_{\text{Lip}}}

% Half rectangle:
\newcommand{\halfrect}[2]{[\![#1,#2)\hspace{-1pt}\!)}
\newcommand{\Rint}{\text{(R)}\int}

% Paired delimiters:
\DeclarePairedDelimiter\parens{(}{)}             % Parentheses
\DeclarePairedDelimiter\sbrac{[}{]}              % Square brackets
\DeclarePairedDelimiter\cbrac{\{}{\}}            % Curly braces
\DeclarePairedDelimiter\set{\{}{\}}              % Set
\DeclarePairedDelimiter\lra{\langle}{\rangle}    % Angle brackets
\DeclarePairedDelimiter\dlra
    {\langle\!\langle}{\rangle\!\rangle}         % Double angle brackets
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}  % Floor
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}     % Ceil
\DeclarePairedDelimiter\norm{\|}{\|}             % Norm
\DeclarePairedDelimiter\abs{|}{|}                % Absolute value

% Shortcuts for angle brackets:
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\lla}{\left\langle}
\newcommand{\rra}{\right\rangle}

% Other commands:
\newcommand{\resp}[1]{[#1]}                  % Respective statement
\newcommand{\bs}{\textbackslash}             % Blackslash in text
% Use \cref in a title.
\newcommand{\creftitle}[2]{\texorpdfstring{\cref{#2}}{#1 \ref{#2}}}
\newcommand{\mcheckthis}{{}^{[\checkmark]}}  % Checkmark in math
\newcommand{\checkthis}{$\mcheckthis$}       % Checkmark in text

% Compatibility with old commands:
\newcommand{\id}[1]{\sd{#1}}
\newcommand{\sargmax}[1]{\argmin_{#1}}
\newcommand{\sargmin}[1]{\argmax_{#1}}
\newcommand{\lrset}[1]{\set*{#1}}
\newcommand{\middleCond}{\middlecond}
\newcommand{\rel}[2]{($(#1) + (#2)$)}
\newcommand{\blackLinks}{}
\newcommand{\Ac}{\A}


\usepackage{xcolor}
\definecolor{mygreen}{HTML}{3C8031}
\definecolor{myred}{HTML}{B6321C}


\definecolor{tab:blue}{HTML}{1F77B4}
\definecolor{tab:orange}{HTML}{FF7F0E}
\definecolor{tab:purple}{HTML}{9467BD}


% \newcommand{\good}{{\color{mygreen} \ding{51}}}
% \newcommand{\bad}{{\color{myred} \ding{55}}}

\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

\newcommand{\bmx}{\mathbf{x}}
\newcommand{\bmy}{\mathbf{y}}

\newcommand{\bmxc}{\mathbf{x}_c}
\newcommand{\bmyc}{\mathbf{y}_c}

\newcommand{\bmxt}{\mathbf{x}_t}
\newcommand{\bmyt}{\mathbf{y}_t}
\newcommand{\pgt}{p_{\text{true}}}

% Neural processes
\DeclareMathOperator{\enc}{enc}
\DeclareMathOperator{\dec}{dec}

==> results/synthetic_tables_average.tex <==
\small
\scshape
\caption{Average Kullback--Leibler divergences in the synthetic Gaussian experiments and average log-likelihoods in the synthetic non-Gaussian experiments.}
\centerline{
\begin{tabular}[t]{lcccccc} 
\toprule 
Gaussian & Int. (1D) & Int. Bd (1D) & Extr. (1D) & Int. (2D) & Int. Bd (2D) & Extr. (2D) \\ \midrule 
FullConvGNP & $\hphantom{-}\mathbf{0.01} { \pm \small 0.00 }$ & $\hphantom{-}\mathbf{0.01} { \pm \small 0.00 }$ & $\hphantom{-}\mathbf{0.00} { \pm \small 0.00 }$ &  &  &  \\ 
\textbf{ConvCNP (AR)} & $\hphantom{-}0.03 { \pm \small 0.00 }$ & $\hphantom{-}0.03 { \pm \small 0.00 }$ & $\hphantom{-}0.02 { \pm \small 0.00 }$ & $\hphantom{-}\mathbf{0.03} { \pm \small 0.00 }$ & $\hphantom{-}\mathbf{0.03} { \pm \small 0.00 }$ & $\hphantom{-}\mathbf{0.02} { \pm \small 0.00 }$ \\ 
ConvGNP & $\hphantom{-}0.04 { \pm \small 0.00 }$ & $\hphantom{-}0.04 { \pm \small 0.00 }$ & $\hphantom{-}1.75 { \pm \small 0.12 }$ & $\hphantom{-}0.12 { \pm \small 0.00 }$ & $\hphantom{-}0.12 { \pm \small 0.00 }$ & $\hphantom{-}0.71 { \pm \small 0.03 }$ \\ 
AGNP & $\hphantom{-}0.10 { \pm \small 0.00 }$ & $\hphantom{-}4.34 { \pm \small 0.17 }$ & $\hphantom{-}5.45 { \pm \small 0.23 }$ & $\hphantom{-}0.17 { \pm \small 0.00 }$ & $\hphantom{-}0.62 { \pm \small 0.01 }$ & $\hphantom{-}0.39 { \pm \small 0.01 }$ \\ 
ConvNP (ELBO) & $\hphantom{-}0.19 { \pm \small 0.01 }$ & $\hphantom{-}0.19 { \pm \small 0.01 }$ & $\hphantom{-}0.29 { \pm \small 0.03 }$ & $\hphantom{-}0.39 { \pm \small 0.01 }$ & $\hphantom{-}0.39 { \pm \small 0.01 }$ & $\hphantom{-}0.36 { \pm \small 0.01 }$ \\ 
\textbf{ACNP (AR)} & $\hphantom{-}0.24 { \pm \small 0.01 }$ & $\hphantom{-}1.08 { \pm \small 0.02 }$ & $\hphantom{-}0.86 { \pm \small 0.01 }$ & $\hphantom{-}0.13 { \pm \small 0.00 }$ & $\hphantom{-}0.57 { \pm \small 0.01 }$ & $\hphantom{-}0.40 { \pm \small 0.01 }$ \\ 
GNP & $\hphantom{-}0.25 { \pm \small 0.01 }$ & F & F & $\hphantom{-}0.25 { \pm \small 0.01 }$ & $\hphantom{-}0.75 { \pm \small 0.01 }$ & $\hphantom{-}0.57 { \pm \small 0.00 }$ \\ 
ConvNP (ML) & $\hphantom{-}0.31 { \pm \small 0.01 }$ & $\hphantom{-}0.31 { \pm \small 0.01 }$ & $\hphantom{-}0.64 { \pm \small 0.01 }$ & $\hphantom{-}0.28 { \pm \small 0.01 }$ & $\hphantom{-}0.28 { \pm \small 0.01 }$ & $\hphantom{-}0.36 { \pm \small 0.01 }$ \\ 
\textit{Diagonal GP} & $\hphantom{-}0.42 { \pm \small 0.02 }$ & $\hphantom{-}0.42 { \pm \small 0.02 }$ & $\hphantom{-}0.84 { \pm \small 0.01 }$ & $\hphantom{-}0.29 { \pm \small 0.01 }$ & $\hphantom{-}0.29 { \pm \small 0.01 }$ & $\hphantom{-}0.40 { \pm \small 0.01 }$ \\ 
ANP (ML) & $\hphantom{-}0.43 { \pm \small 0.01 }$ & $\hphantom{-}1.03 { \pm \small 0.02 }$ & $\hphantom{-}0.78 { \pm \small 0.01 }$ & $\hphantom{-}0.31 { \pm \small 0.01 }$ & $\hphantom{-}0.55 { \pm \small 0.01 }$ & $\hphantom{-}0.39 { \pm \small 0.01 }$ \\ 
ConvCNP & $\hphantom{-}0.43 { \pm \small 0.02 }$ & $\hphantom{-}0.43 { \pm \small 0.02 }$ & $\hphantom{-}0.84 { \pm \small 0.01 }$ & $\hphantom{-}0.30 { \pm \small 0.01 }$ & $\hphantom{-}0.30 { \pm \small 0.01 }$ & $\hphantom{-}0.40 { \pm \small 0.01 }$ \\ 
\textbf{CNP (AR)} & $\hphantom{-}0.46 { \pm \small 0.01 }$ & F & F & $\hphantom{-}0.36 { \pm \small 0.01 }$ & F & F \\ 
NP (ELBO) & $\hphantom{-}0.51 { \pm \small 0.01 }$ & F & $\hphantom{-}4.34 { \pm \small 0.76 }$ & $\hphantom{-}0.40 { \pm \small 0.01 }$ & $\hphantom{-}3.03 { \pm \small 1.68 }$ & $\hphantom{-}0.60 { \pm \small 0.01 }$ \\ 
NP (ELBO, ML) & $\hphantom{-}0.52 { \pm \small 0.02 }$ & F & $\hphantom{-}2.39 { \pm \small 0.33 }$ & $\hphantom{-}0.39 { \pm \small 0.01 }$ & $\hphantom{-}2.35 { \pm \small 1.06 }$ & $\hphantom{-}0.57 { \pm \small 0.01 }$ \\ 
ANP (ELBO, ML) & $\hphantom{-}0.53 { \pm \small 0.01 }$ & $\hphantom{-}1.12 { \pm \small 0.03 }$ & $\hphantom{-}0.85 { \pm \small 0.02 }$ & $\hphantom{-}0.42 { \pm \small 0.01 }$ & $\hphantom{-}0.78 { \pm \small 1.72 }$ & $\hphantom{-}0.41 { \pm \small 0.01 }$ \\ 
ACNP & $\hphantom{-}0.54 { \pm \small 0.02 }$ & $\hphantom{-}1.11 { \pm \small 0.02 }$ & $\hphantom{-}0.84 { \pm \small 0.01 }$ & $\hphantom{-}0.34 { \pm \small 0.01 }$ & $\hphantom{-}0.57 { \pm \small 0.01 }$ & $\hphantom{-}0.40 { \pm \small 0.01 }$ \\ 
ANP (ELBO) & $\hphantom{-}0.54 { \pm \small 0.01 }$ & $\hphantom{-}1.60 { \pm \small 0.06 }$ & $\hphantom{-}1.25 { \pm \small 0.03 }$ & $\hphantom{-}0.43 { \pm \small 0.01 }$ & $\hphantom{-}1.06 { \pm \small 3.04 }$ & $\hphantom{-}0.42 { \pm \small 0.01 }$ \\ 
NP (ML) & $\hphantom{-}0.59 { \pm \small 0.01 }$ & F & $\hphantom{-}1.13 { \pm \small 0.01 }$ & $\hphantom{-}0.41 { \pm \small 0.01 }$ & $\hphantom{-}0.88 { \pm \small 0.03 }$ & $\hphantom{-}0.52 { \pm \small 0.01 }$ \\ 
CNP & $\hphantom{-}0.63 { \pm \small 0.01 }$ & F & $\hphantom{-}1.08 { \pm \small 0.02 }$ & $\hphantom{-}0.43 { \pm \small 0.01 }$ & $\hphantom{-}1.16 { \pm \small 0.45 }$ & $\hphantom{-}0.52 { \pm \small 0.01 }$ \\ 
\textit{Trivial} & $\hphantom{-}1.08 { \pm \small 0.01 }$ & $\hphantom{-}1.08 { \pm \small 0.01 }$ & $\hphantom{-}0.85 { \pm \small 0.01 }$ & $\hphantom{-}0.57 { \pm \small 0.01 }$ & $\hphantom{-}0.57 { \pm \small 0.01 }$ & $\hphantom{-}0.40 { \pm \small 0.00 }$ \\ 
ConvNP (EL., ML) & $\hphantom{-}2.01 { \pm \small 0.11 }$ & $\hphantom{-}2.01 { \pm \small 0.11 }$ & $\hphantom{-}5.95 { \pm \small 0.16 }$ & $\hphantom{-}0.44 { \pm \small 0.01 }$ & $\hphantom{-}0.44 { \pm \small 0.01 }$ & $\hphantom{-}0.47 { \pm \small 0.01 }$ \\ 
\bottomrule \\ 
\end{tabular} 
}
\centerline{
\begin{tabular}[t]{lcccccc} 
\toprule 
Non-Gaussian & Int. (1D) & Int. Bd (1D) & Extr. (1D) & Int. (2D) & Int. Bd (2D) & Extr. (2D) \\ \midrule 
\textbf{ConvCNP (AR)} & $\hphantom{-}\mathbf{1.62} { \pm \small 0.04 }$ & $\hphantom{-}\mathbf{1.62} { \pm \small 0.04 }$ & $\hphantom{-}\mathbf{1.33} { \pm \small 0.04 }$ & $\hphantom{-}\mathbf{0.56} { \pm \small 0.03 }$ & $\hphantom{-}\mathbf{0.56} { \pm \small 0.03 }$ & $\hphantom{-}\mathbf{0.29} { \pm \small 0.03 }$ \\ 
ConvNP (ELBO) & $\hphantom{-}\mathbf{1.62} { \pm \small 0.05 }$ & $\hphantom{-}\mathbf{1.61} { \pm \small 0.05 }$ & $\hphantom{-}0.92 { \pm \small 0.04 }$ & $\hphantom{-}0.06 { \pm \small 0.03 }$ & $\hphantom{-}0.06 { \pm \small 0.03 }$ & $-0.62 { \pm \small 0.04 }$ \\ 
ConvNP (ML) & $\hphantom{-}\mathbf{1.57} { \pm \small 0.06 }$ & $\hphantom{-}\mathbf{1.57} { \pm \small 0.06 }$ & $-0.26 { \pm \small 0.03 }$ & $\hphantom{-}0.26 { \pm \small 0.04 }$ & $\hphantom{-}0.26 { \pm \small 0.04 }$ & $-0.70 { \pm \small 0.02 }$ \\ 
ConvGNP & $\hphantom{-}1.43 { \pm \small 0.08 }$ & $\hphantom{-}1.44 { \pm \small 0.06 }$ & $-0.96 { \pm \small 0.12 }$ & $\hphantom{-}0.23 { \pm \small 0.04 }$ & $\hphantom{-}0.23 { \pm \small 0.04 }$ & $-0.79 { \pm \small 0.02 }$ \\ 
FullConvGNP & $\hphantom{-}1.36 { \pm \small 0.08 }$ & $\hphantom{-}1.37 { \pm \small 0.07 }$ & $-0.15 { \pm \small 0.02 }$ &  &  &  \\ 
ConvCNP & $\hphantom{-}1.19 { \pm \small 0.08 }$ & $\hphantom{-}1.20 { \pm \small 0.06 }$ & $-0.68 { \pm \small 0.02 }$ & $\hphantom{-}0.18 { \pm \small 0.05 }$ & $\hphantom{-}0.18 { \pm \small 0.05 }$ & $-0.86 { \pm \small 0.03 }$ \\ 
\textbf{ACNP (AR)} & $\hphantom{-}0.21 { \pm \small 0.03 }$ & $-0.86 { \pm \small 0.03 }$ & $-0.84 { \pm \small 0.02 }$ & $-0.53 { \pm \small 0.02 }$ & $-1.52 { \pm \small 0.10 }$ & $-1.51 { \pm \small 0.09 }$ \\ 
ANP (ELBO, ML) & $\hphantom{-}0.13 { \pm \small 0.04 }$ & $-0.97 { \pm \small 0.04 }$ & $-0.88 { \pm \small 0.04 }$ & $-0.67 { \pm \small 0.03 }$ & $-1.06 { \pm \small 0.62 }$ & $-0.70 { \pm \small 0.03 }$ \\ 
ANP (ELBO) & $\hphantom{-}0.11 { \pm \small 0.04 }$ & F & $-3.04 { \pm \small 0.08 }$ & $-0.68 { \pm \small 0.03 }$ & $-2.59 { \pm \small 7.64 }$ & $-0.75 { \pm \small 0.03 }$ \\ 
AGNP & $-0.12 { \pm \small 0.03 }$ & $-1.18 { \pm \small 0.07 }$ & $-1.64 { \pm \small 0.12 }$ & $-0.55 { \pm \small 0.02 }$ & $-0.79 { \pm \small 0.02 }$ & $-0.76 { \pm \small 0.03 }$ \\ 
ACNP & $-0.17 { \pm \small 0.03 }$ & $-0.84 { \pm \small 0.03 }$ & $-0.86 { \pm \small 0.03 }$ & $-0.60 { \pm \small 0.02 }$ & $-1.50 { \pm \small 0.10 }$ & $-0.73 { \pm \small 0.03 }$ \\ 
ANP (ML) & $-0.17 { \pm \small 0.03 }$ & $-0.69 { \pm \small 0.03 }$ & $-0.68 { \pm \small 0.03 }$ & $-0.53 { \pm \small 0.02 }$ & $-0.74 { \pm \small 0.04 }$ & $-0.69 { \pm \small 0.02 }$ \\ 
NP (ELBO, ML) & $-0.29 { \pm \small 0.02 }$ & F & F & $-0.66 { \pm \small 0.02 }$ & F & $-0.96 { \pm \small 0.03 }$ \\ 
NP (ELBO) & $-0.30 { \pm \small 0.02 }$ & F & F & $-0.66 { \pm \small 0.02 }$ & F & F \\ 
GNP & $-0.37 { \pm \small 0.02 }$ & F & F & $-0.69 { \pm \small 0.02 }$ & $-0.74 { \pm \small 0.04 }$ & $-0.70 { \pm \small 0.03 }$ \\ 
NP (ML) & $-0.48 { \pm \small 0.02 }$ & $-2.90 { \pm \small 0.39 }$ & $-0.81 { \pm \small 0.03 }$ & $-0.62 { \pm \small 0.02 }$ & $-1.50 { \pm \small 0.11 }$ & $-0.75 { \pm \small 0.03 }$ \\ 
\textbf{CNP (AR)} & $-0.65 { \pm \small 0.02 }$ & $-4.14 { \pm \small 7.34 }$ & $-1.23 { \pm \small 0.13 }$ & $-0.69 { \pm \small 0.02 }$ & $-1.05 { \pm \small 0.07 }$ & $-0.72 { \pm \small 0.03 }$ \\ 
CNP & $-0.66 { \pm \small 0.02 }$ & $-1.65 { \pm \small 0.25 }$ & $-0.75 { \pm \small 0.03 }$ & $-0.69 { \pm \small 0.02 }$ & $-1.05 { \pm \small 0.08 }$ & $-0.71 { \pm \small 0.03 }$ \\ 
\textit{Trivial} & $-0.82 { \pm \small 0.00 }$ & $-0.82 { \pm \small 0.00 }$ & $-0.82 { \pm \small 0.00 }$ & $-0.82 { \pm \small 0.00 }$ & $-0.82 { \pm \small 0.00 }$ & $-0.82 { \pm \small 0.00 }$ \\ 
ConvNP (EL., ML) & $-6.57 { \pm \small 3.76 }$ & $-6.68 { \pm \small 3.76 }$ & F & $-0.04 { \pm \small 0.05 }$ & $-0.04 { \pm \small 0.05 }$ & $-1.47 { \pm \small 0.87 }$ \\ 
\bottomrule \\ 
\end{tabular} 
}
\end{table}

